Referring Video Object Segmentation via Language-aligned Track Selection

Referring video object segmentation (RVOS) requires tracking and segmenting an object throughout a video according to a given natural language expression, demanding both complex motion understanding and the alignment of visual representations with language descriptions. Given these challenges, the recently proposed Segment Anything Model 2 (SAM2) emerges as a potential candidate due to its ability to generate coherent segmentation mask tracks across video frames, and provide an inherent spatio-temporal objectness in its object token representations. In this paper, we introduce SOLA (Selection by Object Language Alignment), a novel framework that leverages SAM2 object tokens as compact video-level object representations, which are aligned with language features through a lightweight track selection module. To effectively facilitate this alignment, we propose an IoU-based pseudo-labeling strategy, which bridges the modality gap between SAM2 representations with language features. Extensive experiments show that SOLA achieves state-of-the-art performance on the MeViS dataset and demonstrate that SOLA offers an effective solution for RVOS. Our project page is available at: https://cvlab-kaist.github.io/SOLA.

==> tables/toy_voc.tex <==
\renewcommand{\arraystretch}{1.1} % Reduce row height globally
\setlength{\heavyrulewidth}{0.8pt} % Thickness for \toprule and \bottomrule
\setlength{\lightrulewidth}{0.8pt} % Thickness for \midrule
\setlength{\cmidrulewidth}{0.5pt}  % Thickness for \cmidrule
\setlength{\extrarowheight}{1pt} % Remove extra row height
\setlength{\aboverulesep}{1pt} % Remove space above rules
\setlength{\belowrulesep}{1pt} % Remove space below rules
\setlength{\belowbottomsep}{1pt} % Remove bottom padding
\setlength{\abovetopsep}{1pt} % Remove top padding

\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \smaller[0.8]{
    \begin{tabular}{C{3.5cm}|C{1cm}C{0.8cm}C{0.8cm}}
    \toprule
    Number of training epochs & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{30} & \multicolumn{1}{c}{40} \\
    \midrule
    Accuracy & 79.9 & 84.8 & 85.3  \\
    \bottomrule
    \end{tabular}%
    }}
    \vspace{-5pt}
    \caption{\textbf{Classification results based on object tokens.} The results show the classification accuracy on the PASCAL-VOC dataset when a linear classification head is applied to object tokens. This demonstrates that SAM2’s object tokens contain semantically meaningful information.}
    \label{tab:toy_voc}
    \vspace{-15pt}
\end{table}
